RobustTSF: Towards Theory and Design of Robust Time Series Forecasting with Anomalies

Time series forecasting is an important and forefront task in many real-world applications. However, most of time series forecasting techniques assume that the training data is clean without anomalies. This assumption is unrealistic since the collected time series data can be contaminated in practice. The forecasting model will be inferior if it is directly trained by time series with anomalies. Thus it is essential to develop methods to automatically learn a robust forecasting model from the contaminated data. In this paper, we first statistically define three types of anomalies, then theoretically and experimentally analyze the loss robustness and sample robustness when these anomalies exist. Based on our analyses, we propose a simple and efficient algorithm to learn a robust forecasting model. Extensive experiments show that our method is highly robust and outperforms all existing approaches. The code is available at https://github.com/haochenglouis/RobustTSF.

==> src/regularizer.tex <==
\section{Regularizer from KD improves network robustness}\label{sec4}

 In this section, we show that a regularizer from knowledge distillation (KD) \cite{park2019relational} can well alleviate the over-fitting problem by using the structure of SSL features. 
Different from classical KD settings where the dataset is clean, our analyses aim at regularizing classifiers learned with noisy supervisions by SSL features.
Understanding the working mechanism is important since it may contribute to the community with a new perspective on learning with label noise by distilling information from SSL features.
In the rest of this section, we will first provide theoretical understanding towards the regularizer under label noise, then perform experiments on different settings to test our analyses.

\subsection{Training Framework}

The training framework is shown in Figure \ref{fig_regularizer}, where a new learning path (SSL training) $f\rightarrow h$ is added to be parallel to Path-2 $f\rightarrow g$ (SL-training) in Figure~\ref{fig:learn_path}.
The newly added \emph{projection head} $h$ is one-hidden-layer MLP (Multi-Layer Perceptron) whose output represents SSL features (after dimension reduction).
Its output is employed to regularize the output of linear classifier $g$ as ${\sf Reg}(h(f(X)),g(f(X)))$.
InfoNCE from SimCLR \citep{chen2020simple} is adopted for SSL training and CE is for SL training. InfoNCE and CE share a common encoder, inspired by the design of self distillation \citep{zhang2019your}.
The loss function is defined as:
\vspace{-3pt}
\begin{equation}\label{sec_4_loss_all}
    L = \mathbb{E}_{\widetilde{\mathcal D}}
    \left\{
    {\sf CE}(g(f(X)),\widetilde{Y}) + {\sf InfoNCE}(X) + {\sf Reg}(h(f(X)),g(f(X)))
    \right\}
\end{equation}


Intuitively, SL features are supposed to be benefited from the structure information from SSL features, e.g., clusterability \citep{zhu2021clusterability} that instances with similar SSL features should have the same true label and instance with different SSL features should have different true labels. 
Mathematically, let $t_{i} = h(f(x_{i}))$, $s_{i}=g(f(x_{i}))$ and $\mathcal{X}^{N}$ to be the set of $N$ tuples of data samples. The distance between $t_{i}$ and $t_{j}$ can be represented as $\phi^{w}(t_{i},t_{j}) = \frac{1}{m}\|t_{i}-t_{j}\|^w$,
where $w\in\{1,2\}$ and $m$ is a normalization term:
\begin{equation}\label{sec4_eq_norm}
m = \frac{1}{|\mathcal{X}^{2}|}\sum_{(x_{i},x_{j}) \in \mathcal{X}^{2}}|| t_{i} - t_{j}||^{w}.
\end{equation}
Then the expectation of ${\sf Reg}(h(X),g(X))$ in Equation (\ref{sec_4_loss_all}) can be estimated by:%
\begin{equation}\label{sec4_eq_reg}
    \mathbb{E}_{X} \left[{\sf Reg}(h(X),g(X)) \right]\approx \frac{1}{|\mathcal{X}^{2}|} \sum_{(x_{i},x_{j}) \in \mathcal{X}^{2}} d(\phi^{w}(t_{i},t_{j}),\phi^{w}(s_{i},s_{j}))
\end{equation}





\begin{figure}[!t]
    \begin{picture}(0,80)(-21,30)
	\centering
	\includegraphics[width = 0.9\textwidth]{fig/regularizer.pdf}
	\end{picture}
	\caption{In this training framework, we adopt CE for SL training and InfoNCE for SSL training. During training, SSL features are utilized to perform regularization on SL features.
	}
	\label{fig_regularizer}
\end{figure}



where $d(\cdot)$ is a distance measure for two inputs.
Popular choices are $l_{1}$, $l_{2}$ or square $l_{2}$ distance. 

\subsection{Analytical Framework}
Under the label noise setting, denote by $d_{i,j} = d(\phi^{w}(t_{i},t_{j}),\phi^{w}(s_{i},s_{j}))$, we have the following decomposition:
\begin{equation}\label{sec4_eq_reg_all}
    \frac{1}{|\mathcal{X}^{2}|} \sum_{(x_{i},x_{j}) \in \mathcal{X}^{2}} d_{i,j}
    = \frac{1}{|\mathcal{X}^{2}|}
    \Big(
    \underbrace{\sum_{(x_{i},x_{j}) \in \mathcal{X}_{\text{clean}}^{2}} d_{i,j}}_{\text{Term-1}}\\
    +
     \underbrace{\sum_{(x_{i},x_{j}) \in \mathcal{X}_{\text{noisy}}^{2}} d_{i,j}}_{\text{Term-2}}
     +
    \underbrace{\sum_{x_{i} \in \mathcal{X}_{\text{clean}}, x_{j}\in \mathcal{X}_{\text{noisy}}} 2 \cdot d_{i,j}}_{\text{Term-3}}
    \Big).
\end{equation}
where $\mathcal{X} = \mathcal{X}_{\text{clean}} \bigcup \mathcal{X}_{\text{noisy}}$, $\mathcal{X}_{\text{noisy}}$ denotes the set of samples whose labels are flipped.
Note the regularizer mainly works when SSL features ``disagree'' with SL features, i.e., Term-3. 
For further analyses, we write Term-3 in the form of expectation with $d$ chosen as square $l_{2}$ distance, \emph{i.e.}, MSE loss:
\vspace{-1pt}
\begin{equation}\label{eq_Lc}
    L_c = 
    \mathbb E_{X^{\text{clean}},X^{\text{noisy}}}
    \left(
   \frac{||g(f(X^{\text{clean}})) - g(f(X^{\text{noisy}}))||^{1}}{m_{1}}  
    -
    \frac{||h(f(X^{\text{clean}})) - h(f(X^{\text{noisy}}))||^{2}}{m_{2}}
    \right)^{2}
\end{equation}
where $m_{1}$ and $m_{2}$ are normalization terms in Equation (\ref{sec4_eq_norm}).
Note in $L_{c}$, we use $w=1$ for SL features and $w=2$ for SSL features.\footnote{Practically, different choices make negligible effects on performance. See more details in Appendix.}  
Denote the variance by ${\sf var}(\cdot)$.
Define notations: 
$$X_+^{\text{noisy}} := X|(\widetilde{Y}=1,Y=0), \quad
X_-^{\text{noisy}} := X|(\widetilde{Y}=0,Y=1).$$
To theoretically measure and quantify how feature correction relates to network robustness, we make three assumptions as follows:
\begin{ap}[Memorize clean instances]\label{fit_clean}
$\forall n \in \{n|\tilde y_n = y_n\}, {\sf CE}(g(f(x_{n})),y_{n}) = 0$.
\end{ap}

\begin{ap}[Same overfitting]\label{var_noisy}
${\sf var}(g(f(X_+^{\text{noisy}})))= 0$ and  ${\sf var}(g(f(X_-^{\text{noisy}}))) =  0$.
\end{ap}

\begin{ap}[Gaussian-distributed SSL features]\label{sec4_assum_gaussian}
The SSL features follow Gaussian distributions, i.e., $h(f(X_{+1})) \sim \mathcal{N}(\mu_{1},\Sigma)$ and $h(f(X_{-1})) \sim \mathcal{N}(\mu_{2},\Sigma)$.
\end{ap}

Assumption \ref{fit_clean} implies that a DNN has confident predictions on clean samples.
Assumption \ref{var_noisy} implies that a DNN has the same degree of overfitting for each noisy sample. For example, an over-parameterized DNN can memorize all the noisy labels \citep{zhang2016understanding,liu2021understanding}. Thus these two assumptions are reasonable. 
Assumption~\ref{sec4_assum_gaussian} follows Assumption~\ref{sec3_assum_1}.
Note in Figure~\ref{fig_regularizer}, SSL features are from $h(f(X))$ rather than $f(X)$. 



\subsection{Theoretical Understanding}
Based on Assumptions~\ref{fit_clean}--\ref{sec4_assum_gaussian}, we
present Theorem \ref{sec4_theom1} to analyze the effect of $L_{c}$.
Recall $X_+^{\text{noisy}} := X|(\widetilde{Y}=1,Y=0),
X_-^{\text{noisy}} := X|(\widetilde{Y}=0,Y=1).$



\begin{thm}\label{sec4_theom1}
When $e_{-} = e_{+}$ and $\mathbb P(Y=1) = \mathbb P(Y=0)$, minimizing $L_{c}$ respect to $g(f(X^{\emph{\text{noisy}}}))$ on DNN results in the following solutions:
\begin{equation*}
    \mathbb{E}_{\substack{X_+^{\emph{\text{noisy}}}}} \left[ g(f(X_+^{\emph{\text{noisy}}})) \right]  = \frac{1}{2} - \frac{1}{2+\Delta(\Sigma,\mu_1,\mu_2)},~
    \mathbb{E}_{\substack{X_-^{\emph{\text{noisy}}}}} \left[ g(f(X_-^{\emph{\text{noisy}}})) \right]  = \frac{1}{2} + \frac{1}{2+\Delta(\Sigma,\mu_1,\mu_2)}, 
\end{equation*}
where $\Delta(\Sigma,\mu_1,\mu_2) := {8\cdot tr(\Sigma)}/{||\mu_{1}-\mu_{2}||^{2}}$, $tr(\cdot)$ denotes the matrix trace, .
\end{thm}






Theorem~\ref{sec4_theom1} reveals a clean relationship between the quality of SSL features (given by $h(f(X))$) and the network robustness on noisy samples.
Note the true label for $X_+^{\text{noisy}}$ is $0$ and the true label for $X_-^{\text{noisy}}$ is $1$. Theorem~\ref{sec4_theom1} shows the regularizer is leading the classifier to predict the feature with corrupted label to its corresponding true label, and the guidance is particularly strong when $\Delta(\Sigma,\mu_1,\mu_2) \rightarrow 0$, e.g., $tr(\Sigma) \rightarrow 0$ or $\|\mu_{1} - \mu_{2}\| \rightarrow \infty$, such that $ \mathbb{E}_{\substack{X_+^{{\text{noisy}}}}}[g(f(X_+^{{\text{noisy}}}))]\rightarrow 0$ and $ \mathbb{E}_{\substack{X_-^{{\text{noisy}}}}}[g(f(X_-^{{\text{noisy}}}))]\rightarrow 1$. Beyond this ideal case, we discuss more interesting findings as:
\squishlist
\item \textbf{Worst case:} The regularizer can always have a positive effect to avoid memorizing wrong labels as long as the model $f\circ h$ is better than randomly initialized models. This is because $\Delta(\Sigma,\mu_1,\mu_2)>0$ when $\mu_1$ and $\mu_2$ are different, and the regularizer is leading the classifier to the true direction when $\Delta(\Sigma,\mu_1,\mu_2)>0$.
\item \textbf{Practical case:}
The model $f\circ h$ is always better than randomly initialized models since SL training can guarantee the performance of encoder $f$ on clean instances, which may generalize to noisy instances, and SSL training can further improve the quality of $f \circ h$.
Thus in practical cases, using SSL features to regularize learning with noisy labels is always beneficial.
\item \textbf{More possibilities:}
Note the proof of Theorem~\ref{sec4_theom1} does not rely on any SSL training process.
From our first finding, we know any encoder helps if it is better than random models.
This makes it possible to use some pre-trained encoders from other tasks.



\squishend







\textbf{High-level understanding on structure regularization:} Even though we have built Theorem \ref{sec4_theom1} to show SL features can benefit from the structure of SSL features by performing regularization, there still lacks high-level understanding of what the regularization is exactly doing.
Here we provide an insight in Theorem \ref{sec4_theom3}, which shows that the regularization is implicitly maximizing mutual information between SL features and SSL features.


\begin{thm} \label{sec4_theom3}
Suppose there always exists a mapping $\xi$ to map $h(f(X))$ to $g(f(X))$. \emph{I.e.,} $g(f(X)) = \xi(h(f(X)))$. Then minimizing Equation (\ref{sec4_eq_reg}) is implicitly maximizing Mutual Information between $h(f(X))$ and $g(f(X))$. \emph{I.e.,} when Equation (\ref{sec4_eq_reg}) achieves $0$, the mutual information $I(h(f(X)),g(f(X)) )$ achieves maximum. 
\end{thm}
The above results facilitate a better understanding on what the regularizer is exactly doing. Note that Mutual Information itself has several popular estimators \citep{belghazi2018mine, hjelm2018learning}. It is a very interesting future direction to develop regularizes based on MI to perform regularization by utilizing SSL features.





\begin{figure}[!t]
    \begin{picture}(40,100)(40,7)
	\centering
	\includegraphics[width = 1.2\textwidth, height = 4cm]{fig/ce_regularizer.pdf}
	\end{picture}
	\caption{Experiments with respect to the regularizer on CIFAR10. ResNet34 is deployed for all the experiments. (a) (b): Encoder is pre-trained by SimCLR. Symmetric noise rate is 20\% and 40\%, respectively; (c) (d): Encoder is randomly initialized. Symmetric noise rate is 40\% and 60\%, respectively. The value of hyper-parameters and other detailed settings in the experiments are reported in the Appendix.
	}
	\label{fig_ce_regularizer}
\end{figure}

\subsection{Experiments}

We provide experiments on CIFAR10 to verify our theory and analysis. The overall experiments are shown in Figure \ref{fig_ce_regularizer}. In the experiments, Regularizer is added at the very beginning since recent studies show that for randomly initialized network, the model tends to fit clean labels first \citep{arpit2017closer}, and we hope the regularizer can improve the network robustness when DNN begins to fit noisy labels.
From Figure \ref{fig_ce_regularizer} (c) (d), for CE training, the performance first increases then decreases since the network over-fits noisy labels as training proceeds. However, for CE with regularizer, the performance is more stable after it reaches the peak.
For 60\% noise rate, the peak point is also much higher than vanilla CE training. 
For Figure \ref{fig_ce_regularizer} (a) (b), since the network is not randomly initialized, it over-fits noisy labels at the very beginning and the performance gradually decreases. However, for CE with regularizer, it can help the network gradually increase the performance as the network reaches the lowest point (over-fitting state). This observation supports Theorem \ref{sec4_theom1} that the regularizer can prevent DNN from over-fitting to noisy labels. More experiments and ablation studies can be found in the Appendix.

==> src/robustce.tex <==
\section{Robustness of Cross-Entropy with SSL Features}\label{sec3}





\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{fig/whycerobust.pdf}
    \caption{Illustration of different learning paths.}
    \label{fig:learn_path}
\end{figure}




We will analyze the robustness of Cross-Entropy with SSL features by comparing three different learning paths as illustrated in Figure~\ref{fig:learn_path}.
Path-1 is the traditional learning path that learns both encoder $f$ and linear classifier $g$ at the same time. Path-2 is the strategy applied in \citep{ghosh2021contrastive} that firstly pre-trains encoder $f$ with SSL, then treats the pre-trained model as a network initialization and jointly fine-tunes $f$ and $g$.
Path-3 is an alternate SSL-based path that first learns the encoder $f$ then only fine-tunes the linear classifier $g$ with fixed $f$.


\subsection{Theoretical Tools}


We prepare some theoretical tools for our analyses.
Our first theorem focuses on demonstrating the effectiveness of only fine-tuning linear classifier $g$ as in Path-3. We present Theorem~\ref{sec3_theom1} below.

\begin{thm} \label{sec3_theom1}
Let $g_{1} = \arg\min_{g \in \mathcal G} \mathbb{E}_{\mathcal D}[{\sf CE}(g(f(X)),Y)]$, $g_{2} =  \arg\min_{g \in \mathcal G} \mathbb{E}_{\widetilde{\mathcal D}}[{\sf CE}(g(f(X)),\widetilde{Y})]$. Then if $e_{+} = e_{-} < 0.5$, we have:
\begin{equation}\label{sec3_eq1}
    {\sf Round}(g_{1}(f(X))) ={\sf Round} (g_{2}(f(X)))
\end{equation}
where $f$ is the fixed encoder and $g$ is the linear classifier, $g(f(\cdot))$ denotes the output whose value ranges from 0 to 1. {\sf Round}$(p)$ is a predictor function that outputs $1$ if $p > 0.5$ and outputs $0$ otherwise.
\end{thm}




Theorem~\ref{sec3_theom1} shows 
with balanced error rates, simply fine-tuning a linear classifier $g$ on the noisy data distribution $\widetilde{\mathcal{D}}$ 
can achieve the same decision boundary as the optimal linear classifier obtained from the corresponding clean distribution $\mathcal D$. \emph{i.e.,} $g_1(f)$ and $g_2(f)$ have the same predictions for all the samples. Theorem~\ref{sec3_theom1} can be generalized to the case with an arbitrary classifier beyond linear. However, admittedly with limited data, training complicated classifiers is hard to converge to the optimal decision boundary. We defer more details to the next subsection.


We then evaluate the former part of Path-3, i.e., the performance of SSL.
Recall in Section~\ref{sec:pre}, SSL is usually evaluated by performance gap between $f\circ g^{\text{Bayes}}$ and $C^{\text{Bayes}}$, where $g^{\text{Bayes}}$ is the optimal linear classifier trained on $\mathcal D$, $f \circ g^{\text{Bayes}}$ denotes the joint model given by $g^{\text{Bayes}}(f(X))$.
We consider a tractable case in Assumption~\ref{sec3_assum_1}.


\begin{ap}\label{sec3_assum_1}
The encoder outputs $f(X_+)$ and $f(X_-)$ follow Gaussian distribution with parameters  $(\mu_{1},\Sigma)$ and $(\mu_{2},\Sigma)$, where $\Sigma = \sigma^{2} \cdot I$, $I$ is the identity matrix.
\end{ap}

\begin{figure}[!t]
    \begin{picture}(100,100)(40,7)

	\centering
	\includegraphics[width = 1.2\textwidth]{fig/tsne.pdf}
	\end{picture}

	\caption{Tsne visualization of the self-supervised encoder outputs $f(X)$  on DogCat \citep{dogcat}, CIFAR10 and CIFAR100 \citep{cifar10}. Different colors stand for different classes.  SimCLR \citep{chen2020simple} is selected for SSL training. Quality of encoders: $(a) \succ (b) \succ (c)$.
	}
	\label{fig_tsne}
\end{figure}

Assumption~\ref{sec3_assum_1} states that the self-supervised features for each class follow simple Gaussian distributions.
We check the effectiveness of this assumption by Figure \ref{fig_tsne}.
It can be observed that the features of each class may have overlapped, but a good SSL method is supposed to return features with good separations (small overlaps).
In Assumption~\ref{sec3_assum_1}, we use $||\mu_{1}-\mu_{2}||$ and $\sigma$ to capture the overlapping area of two classes. If $||\mu_{1}-\mu_{2}||$ is large and $\sigma$ is small, then there exists small overlapping.
Based on this assumption, we show the performance of SSL in Theorem~\ref{sec3_theom2}. 





\begin{thm}\label{sec3_theom2}

If $\mathbb P(Y=1) = \mathbb P(Y=0)$, the risk (error rate) of Bayes optimal classifier $f\circ g^{\emph{\text{Bayes}}}$ follows as:
\begin{equation}
R(f\circ g^{\emph{\text{Bayes}}}) = 1- \varPhi\left(\frac{||\mu_{1} - \mu_{2}||}{2 \cdot \sigma}\right)
\end{equation}
where $\varPhi$ is the cumulative distribution function (CDF) of the standard Gaussian distribution.
\end{thm}



\textbf{Wrap-up~}
With Theorem \ref{sec3_theom1}, we know CE is robust, the performance of which is subject to $f$. Theorem \ref{sec3_theom2} implies that if SSL features learned by $f$ exhibit good property, \emph{i.e.,} when $||\mu_{1} - \mu_{2}||$ is large and $\sigma$ is small, only fine-tuning $g$ can approach the Bayes optimal classifier $C^{\text{Bayes}}$. Therefore, good SSL features induce high performance. In summary, Theorem \ref{sec3_theom1} and Theorem \ref{sec3_theom2} connect SSL features with robustness and generalization ability of CE loss, providing insight on why SSL features improve classification with label noise.  


\subsection{Can We Fix the Encoder?}


We compare the performance of Path-2 with Path-3 in this subsection. 

\subsubsection{Theoretical Analyses~} 
Denote by ${\sf VC}(\mathcal G)$ the VC-dimension of $\mathcal G$. 

\textbf{Always fix good encoders~}
When we fine-tune $g$ on fixed $f$, the learning errors will come from two parts: the encoder error and the classification error.
The encoder error is bounded in Theorem~\ref{sec3_theom2}.
Noting that $g\in\mathcal G$ is a linear classifier with relatively low VC-dimension and ${\sf CE}$ is a calibrated and convex function, the optimization can achieve global optimum with enough samples \citep{bartlett2006convexity}, e.g., w.p. $1-\delta$, the learning error will be $\varepsilon$ with $\Theta(\frac{{\sf VC}(\mathcal G)+\ln{1/\delta}}{\varepsilon})$ \emph{i.i.d.} instances \citep{vapnik2013nature}.
Recall Theorem \ref{sec3_theom1} also guarantees the optimality of $g$ learned under the noisy distribution $\widetilde{\mathcal D}$.
Therefore, given a good encoder with large enough $\frac{\|\mu_1-\mu_2\|}{\sigma_1}$, we should keep it fixed since the simple linear classifier $g$ trained under label noise only requires $N=\Theta(\frac{{\sf VC}(\mathcal G)+\ln{1/\delta}}{\varepsilon})$ \emph{i.i.d.} instances in $\widetilde{D}$ to achieve around $\varepsilon$ errors with high probability, which performs well enough to approximate $C^{\text{Bayes}}$.

\textbf{Updating $f$ is not stable~}
If $f$ is unfixed, due to the non-convexity and over-fitting capability of $f$, network trained on vanilla $\widetilde{D}$ will likely and ultimately overfit to noisy labels \citep{zhang2016understanding}, particularly when the number of instances is insufficient. For example, w.p. $1-\delta$, jointly learning $f$ and $g$ and achieving error $\varepsilon$ requires $\Theta(\frac{{\sf VC}(\mathcal F \circ \mathcal G)+\ln{1/\delta}}{\varepsilon})$ \emph{i.i.d.} instances, which is far more than the number required in only tuning $g$ due to the huge capacity of DNNs.
Note the effective \emph{i.i.d.} instances would decrease with the increase of noise rates.
Although a good initialization contributes to better convergence, $f$ will be misled by label noise in extreme cases.
Therefore it is unreasonable to assume that CE will stably induce the network to approximate the Bayes optimal classifier under label noise. In other words, if $f$ is not fixed, due to the overfitting capability of $f$, the outputs of $f(X)$ would be contaminated by the label noise before $g$. In contrast, the original SSL features are independent %
from the label noise if $f$ is fixed. We therefore conclude that CE on vanilla $\widetilde{D}$ is not robust. 
Note \citep{nodet2021contrastive} claimed the encoder should not be fixed during fine-tuning based on some experiments. We include more discussions in Appendix.


\begin{figure}[!t]
    \begin{picture}(40,100)(40,7)
	\centering
	\includegraphics[width = 1.2\textwidth, height = 4cm]{fig/robustce.pdf}
	\end{picture}
	\caption{(a) (b) (c): Performance of CE on DogCat, CIFAR10 and CIFAR100 under symmetric noise rate. For each noise rate, the best epoch test accuracy is recorded. The blue line represents training with fixed encoder and the red line represents training with an unfixed encoder; (d): test accuracy of CIFAR10 on each training epoch under symmetric 0.6 noise rate. We use ResNet50 for DogCat and ResNet34 for CIFAR10 and CIFAR100. SimCLR is used to deploy SSL pre-training. Detailed experimental settings are reported in the Appendix.
	}
	\label{fig_robustce}
\end{figure}
\vspace{-3pt}



\subsubsection{Empirical evidence}
We conduct experiments in Figure \ref{fig_robustce} to support our theorems and analyses above. 

\textbf{Overall performance~}
From Figure \ref{fig_robustce}(a)--(c), when  encoder $f$ is fixed, the performance of CE (fixed encoder) exhibits great robustness as the noise rate increases and only has a little drop when the symmetric noise rate approximates the maximum theoretical value for each dataset (0.5 for DogCat, 0.9 for CIFAR10) which verifies Theorem \ref{sec3_theom1} and Theorem \ref{sec3_theom2}. Note that the drop is because, to reach the condition specified in Equation (\ref{sec3_eq1}), a substantial number of training samples are needed. %
However, for example, each class only has 500 samples in CIFAR100. As the noise rate increases, the number of clean samples will further decrease which makes the classifier hard to learn from the distribution. 

\textbf{Fixed encoder benefits extreme label noise~}
Next, we observe the
 the performance gap between SSL and SL when datasets are clean. This gap can be visualized in  Figure \ref{fig_robustce} (a) (b) (c) at $\text{noise rate} = 0$. For DogCat, the gap is very small, thus CE with fixed encoder always exhibits better performance. For CIFAR10, the gap is moderate, the performances of CE (fixed encoder) and CE (unfixed encoder) are close when noise rate is small. However, when noise rate is high, CE with fixed encoder still exhibits better performance. For CIFAR100, the gap is large, thus CE with fixed encoder shows better performance only when noise rate is over 0.7. 
 
\textbf{Fixed encoder has better convergence~}
 Note that the performance in Figure \ref{fig_robustce} (a) (b) (c) is selected from best epoch accuracy. If we take the last epoch accuracy into consideration. CE with fixed encoder has great advantage over unfixed encoder. Figure \ref{fig_robustce} (d) depicts the performance of CE in terms of training epochs under 0.6 symmetric noise rate on CIFAR10. We find that even though these two approaches have almost same best epoch accuracy, CE with fixed encoder is more robust as training proceeds. For CE with unfixed encoder, since the self-supervised pre-trained network's weights serve as a better initialization, it shows good performance in the beginning. However, because of the memorizing effect of DNN, it will still over-fit to noisy labels in the end.%



\textbf{Generalize to class- and instance-dependent label noise:} 
Theorem \ref{sec3_theom1} shows that CE is robust to label noise when $e_- = e_+$. However, for a more general label noise such as asymmetric class-dependent label noise or instance-dependent label noise, CE with fixed encoder on vanilla $(f(X),\widetilde{Y})$ is hard to be guaranteed to be robust because for instance noise, noise rate varies for each class. But it does not mean SSL features can not help.  We may still fix the encoder and perform a simple down-sampling to balance the noisy dataset before fine-tuning the linear classifier.
For example, for class-dependent label noise that is not symmetric, the down-sampling is conducted to make $\mathbb P(\widetilde{Y}=i) = \mathbb P(\widetilde{Y}=j)$ in the noisy dataset which can well approximate the condition in Theorem \ref{sec3_theom1} (Illustration is deferred to Appendix).
Although not theoretically guaranteed, similar down-sampling strategy should also benefit the learning with instance-dependent label noise, which may be highly unbalanced.
We perform an experiment in Table \ref{table:instance} to verify the effectiveness of the down-sampling in the setting of instance-dependent label noise (generation of label noise is followed by \citep{sieve2020}).
From the experiments, if no sampling strategy is conducted, CE with fixed encoder does not show many benefits. In some cases, it even performs worse than CE baseline (unfixed $f$ with random init). However, with down-sampling, CE with fixed encoder even outperforms CORES \citep{sieve2020} by a large margin. Even though our main purpose in the paper is not to develop new methods for achieving SOTA, we think this down-sampling strategy motivated by Theorem \ref{sec3_theom1} can inspire further research on instance-dependent label noise by using SSL features.

\begin{table*}[!t]
		\caption{Comparison of test accuracies of each method under instance-based label noise. CE (unfixed $f$ with random init.) is a common baseline adopted in the literature which trains a random initialized DNN using CE loss on noisy dataset. }
		\begin{center}
			\footnotesize{\begin{tabular}{c|cccccc} 
				\hline 
				 \multirow{2}{*}{Method}  & \multicolumn{3}{c}{\emph{Inst. CIFAR10} } & \multicolumn{3}{c}{\emph{Inst. CIFAR100} }   \\ 
				 & $\varepsilon = 0.2$&$\varepsilon = 0.4$&$\varepsilon = 0.6$ & $\varepsilon = 0.2$&$\varepsilon = 0.4$&$\varepsilon = 0.6$\\
				\hline\hline
			      CORES \citep{sieve2020} &89.50 &82.84 & 79.66  & 61.25 & 47.81 &37.85\\
			       CE (unfixed $f$ with random init.)&87.16&75.16 & 44.64 &58.72 & 41.14 & 25.29\\
				 CE (fixed $f$, no sampling) &88.74 & 75.71 & 25.7 & 59.38 & 46.13  &24.75\\
				CE (fixed $f$, down-sampling)  &\textbf{90.12} & \textbf{84.19} & \textbf{82.06} & \textbf{62.88} & \textbf{61.1}  &\textbf{58.93}\\
			   \hline
			\end{tabular}}
		\end{center}
		\vspace{-5pt}
		\label{table:instance}
	\end{table*}


\subsection{Takeaways}

Our both theoretical and empirical results demonstrate that: We need to simply fix the encoder when 1) the encoder is sufficiently good, 2) the high noise rate decreases the number of effective \emph{i.i.d.} instances to a certain level, 3) the over-parameterized model makes it easy to overfit label noise.
However, there are some concerns: 1) If the gap between SL and SSL is relatively large, CE with unfixed encoder has more advantage on small noise rate (e.g., Figure~\ref{fig_robustce} (c)); 2) Consider an online classification system which always needs new training data to update itself. If we only fine-tune the linear classifier for keeping robustness to label noise, then due to the limited learnability of affine functions, this online classification system may learn very limited knowledge from unseen data.
Therefore, it is necessary to update the encoder while keeping it stable and robust to label noise, which is the focus in the next section.























